Retrieval Augmented Generation for Dynamic Graph Modeling

Modeling dynamic graphs, such as those found in social networks, recommendation systems, and e-commerce platforms, is crucial for capturing evolving relationships and delivering relevant insights over time. Traditional approaches primarily rely on graph neural networks with temporal components or sequence generation models, which often focus narrowly on the historical context of target nodes. This limitation restricts the ability to adapt to new and emerging patterns in dynamic graphs. To address this challenge, we propose a novel framework, Retrieval-Augmented Generation for Dynamic Graph modeling (RAG4DyG), which enhances dynamic graph predictions by incorporating contextually and temporally relevant examples from broader graph structures. Our approach includes a time- and context-aware contrastive learning module to identify high-quality demonstrations and a graph fusion strategy to effectively integrate these examples with historical contexts. The proposed framework is designed to be effective in both transductive and inductive scenarios, ensuring adaptability to previously unseen nodes and evolving graph structures. Extensive experiments across multiple real-world datasets demonstrate the effectiveness of RAG4DyG in improving predictive accuracy and adaptability for dynamic graph modeling. The code and datasets are publicly available at https://github.com/YuxiaWu/RAG4DyG.

==> app.tex <==
\section*{Appendix}


 




\section{Retrieval Data Annotation}
\label{app-anno}

To facilitate retrieval model training, we regard the samples in the training dataset as our retrieval pool $D=\{(x_i, y_i)\}_{i=1}^{M}$ where each pair $(x_i, y_i)$ represents the historical sequence and its corresponding target sequence. Specifically, $x_i$ is the input sequence before the last time step and $y_i$ is the output sequence at the last time step. We annotate demonstrations based on the Jaccard similarity of $y_i$ among all the pairs in $D$.

\begin{equation}
    r(y_i,y_j) = \frac{|y_i \cap y_j|}{|y_i \cup y_j|}
\end{equation}

 To control the quality of annotated data, we set a threshold of 0.8 to select highly similar demonstrations for each sample. These filtered annotations are then used to train the retriever model. The number of training samples for UCI, Hepth, MMConv, Wikipedia and Enron datasets are 9,578, 8,250, 10,762, 162,408 and 2,510,666 respectively. \textcolor{blue}{todo: reddit}


\section{More Details about Baselines}
\label{app-baseline}

The details of the baselines are as follows:
\iffalse
%\vspace{-0.1cm}
\begin{itemize}
%\setlength\itemsep{0.3em}
\item \textbf{DySAT} \cite{sankar2020dysat} utilizes self-attention mechanisms to capture both structural and temporal patterns in dynamic graphs through discrete-time snapshots.

\item \textbf{EvolveGCN} \cite{pareja2020evolvegcn}  leverages recurrent neural networks to evolve the graph convolutional network parameters over discrete time steps.

\item \textbf{DyRep} \cite{trivedi2019dyrep} models dynamic graphs in continuous time by incorporating both temporal point processes and structural dynamics to capture interactions and node dynamics.

\item \textbf{JODIE} \cite{kumar2019predicting}  focuses on user and item embedding trajectories over continuous time, predicting future interactions by modeling user and item embeddings jointly.

\item \textbf{TGAT} \cite{xu2020inductive}  employs temporal graph attention layers and time encoding to capture temporal dependencies and structural information for dynamic graphs.

\item \textbf{TGN} \cite{rossi2020temporal} combines GNNs with memory modules to maintain node states over continuous time, effectively learning from dynamic interactions.

\item \textbf{TREND} \cite{wen2022trend} integrates temporal dependencies based on Hawkes process and GNN to learn the dynamics of graphs.


\item \textbf{GraphMixer} \cite{cong2022we} 
introduces a novel architecture that leverages MLP-mixer to learn link-encoder and node encoder for evolving graphs in continuous time.

\item \textbf{SimpleDyG} \cite{wu2024feasibility} reformulated the dynamic graph modeling as a sequence modeling task and mapped the dynamic interactions of target nodes as sequences with specially designed tokens. It simplifies dynamic graph modeling without complex architectural changes to effectively capture temporal dynamics.
\end{itemize}
\else
\section{More Experimental Results }
For the effect of different retrieval methods for generative performance in Sec. 5.3, we report the NDCG@5 score in Table \ref{fusion}. Here we report the remaining metrics in Table \ref{app table: re for gen}. The results show that RAG4DyG performs better than BM25 and Jaccard on Recall@5 and Jaccard metrics, which are consistent with the performance of NDCG@5. 

\begin{table*}[h!]
	\centering
	%\small
	%\addtolength{\tabcolsep}{-4pt}
	%\renewcommand*{\arraystretch}{1}
\setlength{\tabcolsep}{2pt}
\resizebox{0.9\textwidth}{!}{
       %\vspace{-0.1cm}
    	\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
		
		\toprule
		\multicolumn{1}{c|}{\multirow{2}{*}{Method}}& \mc{2}{c|}{UCI} & \mc{2}{c|}{Hepth} & \mc{2}{c|}{MMConv} & \mc{2}{c|}{Wikipedia} & \mc{2}{c}{Enron}\\
		\cmidrule{2-11}
		& {Recall@5}  & {Jaccard}  
        & {Recall@5}   & {Jaccard}   
        & {Recall@5} & {Jaccard}  
        & {Recall@5} & {Jaccard}  
        & {Recall@5} & {Jaccard}  
        \\	
		\midrule		
		
		\textit{BM25}  
           &\textbf{0.111}\scriptsize{±0.007} %&0.121\scriptsize{±0.009}    
           &0.093\scriptsize{±0.004}
           
            & -   & - %&-
            
           &  0.193\scriptsize{±0.003}
           %& 0.207\scriptsize{±0.003}
           &0.192\scriptsize{±0.003}  

           &0.368\scriptsize{±0.01} 
           &0.325\scriptsize{±0.01} 

        & \textbf{0.105}\scriptsize{±0.003} 
        & \textbf{0.075}\scriptsize{±0.002} 
           
           \\ 
        \textit{Jaccard}
           & 0.104\scriptsize{±0.009} 
           %& 0.113\scriptsize{±0.011}    
           & 0.088\scriptsize{±0.010} 
            
            & -  &- %&-
            
         & 0.193\scriptsize{±0.004}  
         %& 0.207\scriptsize{±0.005}
         &0.192\scriptsize{±0.004}

         &0.368\scriptsize{±0.013} 
         &0.321\scriptsize{±0.011} 
         &0.102\scriptsize{±0.004} 
         &0.073\scriptsize{±0.002} 
         
         \\ 
        \textit{RAG4DyG}  
            & \textbf{0.111}\scriptsize{±0.013} 
            %& \textbf{0.122}\scriptsize{±0.014}    
            & \textbf{0.097}\scriptsize{±0.010}  
         
            &\textbf{0.019}\scriptsize{±0.002}    
            %& \textbf{0.045}\scriptsize{±0.003}   
            & \textbf{0.019}\scriptsize{±0.002}
            
            &\textbf{0.194}\scriptsize{±0.005}   
            %& \textbf{0.208}\scriptsize{±0.005}   
            & \textbf{0.194}\scriptsize{±0.005} 

            &\textbf{0.369}\scriptsize{±0.006} 
            &\textbf{0.328}\scriptsize{±0.007} 
            
            &0.1\scriptsize{±0.003}  
            &0.071\scriptsize{±0.002} 
       \\         
         \midrule

         \textit{GroundTruth}  
            & 0.121\scriptsize{±0.010}  
            %& 0.129\scriptsize{±0.010}  
            & 0.107\scriptsize{±0.012}
         
           & 0.028\scriptsize{±0.004}   
           %& 0.062\scriptsize{±0.007}
           &0.028\scriptsize{±0.004}
           
            & 0.210\scriptsize{±0.008}    
            %& 0.224\scriptsize{±0.008}    
            & 0.208\scriptsize{±0.008}  

            &0.39\scriptsize{±0.008}  
            &0.34\scriptsize{±0.006}  
            
            &0.116\scriptsize{±0.002}  
            &0.087\scriptsize{±0.002}  
            
        \\ 
		\bottomrule
	\end{tabular}
 }
	%\vspace{-0.1cm}
\caption{Generative performance of retrieval methods.}
 \label{app table: re for gen}
\end{table*}

For the effect of different fusion strategies in Sec. 5.3, the performance of the remaining metrics is shown in Table \ref{app table: fusion}. Similarly, the ``GraphFusion'' strategy outperforms direct concatenation and ``MLP'', indicating the effectiveness of the graph structure among demonstrations.

\begin{table*}[ht]
	\centering
	%\small
	%\addtolength{\tabcolsep}{-4pt}
	%\renewcommand*{\arraystretch}{1}
\setlength{\tabcolsep}{2pt}
\resizebox{0.9\textwidth}{!}{
       %\vspace{-0.1cm}
    	%\begin{tabular}{@{}c|ccc|ccc|ccc@{}}
    	\begin{tabular}{@{}c|cc|cc|cc|cc|cc@{}}
		
		\toprule
		%\multicolumn{1}{c|}{\multirow{2}{*}{Fusion strategy}}& \mc{3}{c|}{UCI} & \mc{3}{c|}{Hepth} & \mc{3}{c}{MMConv} \\ \cmidrule{2-10}
  	\multicolumn{1}{c|}{\multirow{2}{*}{Fusion strategy}}& \mc{2}{c|}{UCI} & \mc{2}{c|}{Hepth} & \mc{2}{c|}{MMConv}& \mc{2}{c|}{Wikipedia}& \mc{2}{c}{Enron} \\ \cmidrule{2-11}
		%& {Recall@5} & {NDCG@5}     & {Jaccard}   & {Recall@5}  &{NDCG@5} & {Jaccard}  & {Recall@5}   &{NDCG@5} & {Jaccard} \\	
		& {Recall@5}   & {Jaccard}   & {Recall@5}  & {Jaccard}  & {Recall@5}  & {Jaccard} & {Recall@5}  & {Jaccard} & {Recall@5}  & {Jaccard} \\			
		\midrule		

  \textit{Concatenation}  
        & 0.033\scriptsize{±0.019}   
        %& 0.036\scriptsize{±0.018}
        & 0.029\scriptsize{±0.016}
        
        & 0.001\scriptsize{±0.002}  
        %& 0.007\scriptsize{±0.002}  
        & 0.002\scriptsize{±0.002} 
        
        & 0.103\scriptsize{±0.031}  
        %& 0.110\scriptsize{±0.030}  
        & 0.103\scriptsize{±0.031} 
        
        &0.21\scriptsize{±0.019} 
        &0.206\scriptsize{±0.019} 
        
        &0.04\scriptsize{±0.016}
        &0.033\scriptsize{±0.013}
        \\ 
        
    \textit{MLP}  
        & 0.102\scriptsize{±0.018}  
        %& 0.106\scriptsize{±0.017} 
        & 0.089\scriptsize{±0.016}
          
        & 0.006\scriptsize{±0.002}    
        %& 0.015\scriptsize{±0.002} 
        & 0.006\scriptsize{±0.002}
        
        & 0.156\scriptsize{±0.006}  
        %& 0.167\scriptsize{±0.006}   
        & 0.153\scriptsize{±0.006} 
        
        & 0.356\scriptsize{±0.006}  
        & 0.321\scriptsize{±0.007}  
        
        & 0.094\scriptsize{±0.003}  
        & 0.067\scriptsize{±0.002}  
        \\
        
    \textit{GraphFusion}  
          & \textbf{0.111}\scriptsize{±0.013} 
          %& \textbf{0.122}\scriptsize{±0.014}    
          & \textbf{0.097}\scriptsize{±0.010}  
         
         & \textbf{0.019}\scriptsize{±0.002}    
         %& \textbf{0.045}\scriptsize{±0.003 }   
         &  \textbf{0.019}\scriptsize{±0.002} 
          
          & \textbf{0.194}\scriptsize{±0.005}    
          %& \textbf{0.208}\scriptsize{±0.005}   
          & \textbf{0.194}\scriptsize{±0.005} 
          
        & \textbf{0.369}\scriptsize{±0.006}    
        &\textbf{0.328}\scriptsize{±0.007} 
        
        & \textbf{0.1}\scriptsize{±0.003}  
        & \textbf{0.071}\scriptsize{±0.002} 
          \\ 
               
		\bottomrule
	\end{tabular}}
	%\vspace{-0.1cm}
     \caption{Effect of different fusion strategies.}
     \vspace{-2mm}
     \label{app table: fusion}
\end{table*}

\section{Hyper-parameter Settings}
\label{app-para}
\iffalse
We run all the experiments on an NVIDIA GPU L40 with the same data splitting and follow the hyper-parameter settings reported in SimpleDyG  \cite{wu2024feasibility} for all the baselines. For our RAG4DyG method, we report the hyper-parameters as follows.

The time decay rate $\lambda$ for the retrieval model in Eq. (4) was fine-tuned according to the time granularity of different datasets, with days for the UCI dataset, months for the Hepth dataset, and turns for the MMConv dataset. We explored a range of values $\lambda = \{1e-4, 1e-3, 1e-2, 1e-1, 1, 10, 100\}$, ultimately selecting $\lambda = 1e-4$ for UCI, $\lambda = 0.1$ for Hepth, and $\lambda = 10$ for MMConv. The coefficient $\alpha$ in the loss function (Eq. (8) was tuned across $\{0.2, 0.4, 0.6, 0.8, 1\}$, resulting in final values of $\alpha = 1$ for UCI and MMConv dataset, $\alpha = 0.4$ for Hepth. Additional parameter settings for the three datasets are as follows: the temperature $\tau$ in the two contrastive learning tasks is set to $\tau = \{0.1, 0.1, 0.1\}$; the batch size of the retriever model is $N = \{64, 128, 128\}$; and the masking and cropping portions in context-aware contrastive learning are $\{0.8, 0.8, 0.8\}$ and $\{0.4, 0.6, 0.6\}$, respectively.
\else

==> data.tex <==
\section{Data Annotation}

\subsection{Data preprocessing}
\iffalse
\textbf{Recap}: In the SimpleDyG model, we view the interaction of an ego node as a sequence as below:
$$s_i = \langle |history| \rangle, v_i, \langle |time1| \rangle, v_1^{t1}, v_2^{t2}, ..., \langle|timeT-1|\rangle, v_1^{tT-1}, ... \langle |endofhistory| \rangle, \langle |pred| \rangle, v_1^{tT}, ... \langle |endofore| \rangle$$
where $T$ is the time step of prediction.
\fi
In this section, we introduce data preprocessing to train a retriever for dynamic graph modeling by sequences. We use the sequences in the training dataset as the retrieval source. Since our goal is to find the similar cases that have inherent historical interaction pattern and similar behavior in future timestamps, we annotate the dataset based on the similarity of the last timestamp among different samples. For each pair of samples $s_i$ and $s_j$, we define the Jaccard similarity score based on the interactions to be predicted as   

\begin{equation}
    sim_{ij} = \frac{|s_i \cap s_j|}{|s_i \cup s_j|}
\end{equation}

To control the annotation quality, we set a threshold for the similarity score to identify the similar pairs. The statistical information after prepossessing all the datasets is provided in Table.    

==> intro.tex <==




\section{Introduction}

\begin{figure*}[ht] 
\centering
\subfigure[RAG in NLP]{
\centering
    \includegraphics[scale=0.8]{img/RAG-in-NLP.pdf}
    \label{RAG-in-NLP}
}\hspace{8mm}%
\subfigure[RAG in dynamic graphs]{
    \centering
    \includegraphics[scale=0.8]{img/RAG-in-Graph.pdf}
    \label{RAG-in-Graph}
}
%\vspace{-2mm}
 \caption{Illustration of RAG in NLP and dynamic graph modeling. (a) In NLP, RAG leverages pre-trained language models to encode text and retrieve semantically similar or related demonstrations, which are further concatenated to enhance the generation task. (b) Our work addresses the challenges of complex temporal and structural characteristics of dynamic graphs, incorporating RAG through time- and context-aware retrieval and graph fusion modules.}
 %\vspace{-2mm}
 \label{RAG}
\end{figure*}

%Dynamic graphs, which track the temporal evolution of nodes and edges, are essential for analyzing complex systems across domains like social networks, citation networks etc.
Dynamic graph modeling is pivotal in information retrieval, enabling the analysis and prediction of evolving relationships and interactions across applications such as Web search, recommendation systems, and conversational information retrieval.
 Existing methods for dynamic graph modeling fall into two main categories: discrete-time and continuous-time approaches \cite{feng2024comprehensive}. Discrete-time methods divide the timeline into intervals, capturing the graph's state at each point \cite{sankar2020dysat}, but they lack temporal granularity by overlooking event dynamics within intervals. Continuous-time approaches, on the other hand, model temporal dynamics continuously, without discretization, allowing for more detailed representations \cite{trivedi2019dyrep,xu2020inductive, wen2022trend}. Our work aligns with continuous-time approaches, aiming to capture fine-grained time steps for more accurate dynamic graph modeling.

Traditional approaches for dynamic graph modeling predominantly rely on integrating graph neural networks (GNNs) with specialized temporal modules, such as recurrent neural networks \cite{pareja2020evolvegcn}, self-attention \cite{sankar2020dysat} and temporal point processes \cite{wen2022trend}, which update the graph representations over time. Although powerful, these methods suffer from the inherent limitations of GNNs, such as difficulty with long-term dependencies, and over-smoothing or over-squashing issues \cite{chen2020measuring,alon2020bottleneck}. Recently, a simple and effective approach called SimpleDyG \cite{wu2024feasibility} redefines dynamic graph modeling as a generative sequence
modeling task and leverages the strengths of sequence models like Transformers to capture long-range dependencies within temporal sequences effectively. 

Despite significant advancements in dynamic graph modeling, current approaches heavily depend on isolated historical contexts of the target nodes, limiting each node's perspective to its ego network. The limited context makes it difficult to quickly adapt to diverse emerging patterns. For example, in a social network, when users transit to new behavioral patterns or when new users with minimal historical interactions are introduced, traditional models that focus on the historical contexts of individual nodes might not respond effectively to these changes. To overcome these limitations, we draw inspiration from the Retrieval-Augmented Generation (RAG) technique originated from the Natural Language Processing (NLP) field \cite{gao2023retrieval}. As shown in Fig.~\ref{RAG-in-NLP}, RAG broadens the context through the retrieval of additional demonstrations, achieving considerable success in NLP. In this work, we aim to integrate RAG into dynamic graph modeling to incorporate a broader and more relevant contextual understanding beyond the historical interactions of individual nodes. However, leveraging RAG for dynamic graph modeling presents two critical challenges.

First, \textit{how do we harvest high-quality demonstrations for dynamic graphs?}
This involves selecting the most contextually and temporally relevant samples to enrich the current state of a target node. While training-free retrieval methods, such as BM25 \cite{robertson1976relevance, fang2004formal} and other matching-based schemes, 
%or leveraging the overlap ratio of nodes across different sequences, 
offer simplicity and computational efficiency, they struggle to handle inductive scenarios that involve unseen nodes at inference time, as unseen nodes lack historical interactions for effective matching.
%. In such cases, unseen nodes lack historical interactions, limiting the applicability of these methods.} 
Unlike RAG for NLP, where external textual data and a pre-trained language model (LM) naturally support demonstration retrieval as shown in Fig.~\ref{RAG-in-NLP}, dynamic graph modeling requires careful consideration of the data sources and the ability to handle complex structural and temporal patterns as shown in Fig.~\ref{RAG-in-Graph}. To address this, we introduce a novel time-aware contrastive learning strategy that leverages internal training data for demonstration retrieval. 
Following SimpleDyG \cite{wu2024feasibility}, we regard dynamic graph modeling as a sequence modeling task and the prediction of future events as a sequence generation problem. Hence, we define a \emph{query sequence} for a target node as its historical interaction sequence. Next, we automatically annotate the retrieval training pool by assessing the similarity to the query. Given the training pool, our model consists of two contrastive modules: time-aware and context-aware contrastive learning. The former utilizes a time decay function to prioritize samples that are temporally close to the query, while the latter incorporates data augmentation techniques such as masking and cropping to improve the model's ability to retrieve complex structural patterns.

Second, \textit{how do we effectively integrate the retrieved demonstrations into the dynamic graph model?} This involves fusing the retrieved demonstrations to enrich the historical context of each target node and enhance subsequent predictions. Directly concatenating the retrieved demonstrations with the query sequence not only results in a lengthy sequence unsuited for generative predictions but also overlooks the structural patterns among the retrieved demonstrations. To address this, we propose graph fusion, leveraging the graph structures inherent to the demonstrations and fusing them into a summary graph, as shown in Fig.~\ref{RAG-in-Graph}. We then apply a GNN-based readout to learn the representation of the fused summary graph, which is prepended to the query sequence before being fed into the sequence generation model.

Our contributions can be summarized as follows.
%\begin{itemize}
    (1) We propose a novel Retrieval-Augmented Generation approach for Dynamic Graph modeling named RAG4DyG. It employs a retriever to broaden the historical interactions with contextually and temporally relevant demonstrations, leading to enhanced generative predictions on dynamic graphs.
    (2) We propose a time-aware contrastive learning module that incorporates temporal and structural information for demonstration retrieval. Additionally, we design a graph fusion module to effectively integrate the retrieved demonstrations, leveraging structural enhancements for subsequent predictions.  (3) We conduct extensive experiments to validate our approach, demonstrating the effectiveness of RAG4DyG in various domains. 
    %and superiority over existing methods in dynamic graph modeling.
%\end{itemize}





